Agent-based Dynamics of a SPAHR Opioid Model on Social Network Structures

Addiction epidemiology has been an active area of mathematical research in recent years. However, the social and mental processes involved in substance use disorders versus contraction of a pathogenic disease have presented challenges to advancing the epidemiological theory of substance abuse, especially within the context of the opioids where both prescriptions and social contagion have played a major role. In this paper, we utilize an agent-based modeling approach on social networks to further explore these dynamics. Using parameter estimation approaches, we compare our results to that of the Phillips et al. SPAHR model which was previously fit to data from the state of Tennessee. Our results show that the average path length of a social network has a strong relationship to social contagion dynamics for drug use initiation, while other pathways to substance use disorder should not be constrained to social network interactions that predate the individual's drug use.

==> reviewers.tex <==
Richard Larson, rclarson@mit.edu (author on Cutter paper that we cite, which cited us quite positively and pointed out the need for a study just like this one)
Stephen Wirkus, swirkus@asu.edu
Wandi Ding, wding@mtsu.edu (Graduated from UTK, biomath modeler, professor at MTSU, interested in our opioid work and ABMs)
